BeLLM: Backward Dependency Enhanced Large Language Model for Sentence Embeddings

Sentence embeddings are crucial in measuring semantic similarity. Most recent studies employed large language models (LLMs) to learn sentence embeddings. Existing LLMs mainly adopted autoregressive architecture without explicit backward dependency modeling. Therefore, we examined the effects of backward dependencies in LLMs for semantic similarity measurements. Concretely, we propose a novel model: backward dependency enhanced large language model (BeLLM). It learns sentence embeddings via transforming specific attention layers from uni- to bi-directional. We extensively experiment across various semantic textual similarity (STS) tasks and downstream applications. BeLLM achieves state-of-the-art performance in varying scenarios. It shows that auto-regressive LLMs benefit from backward dependencies for sentence embeddings.

==> methodology.old.tex <==
\input{figure_framework}

Our quantitative analysis has revealed the limited capability of LLMs to capture dependencies. Therefore, in this section, we will present our proposed model, BeLLM, for incorporating backward dependencies into LLMs to enhance the capability to capture dependencies. Figure \ref{figure_framework} shows the generic framework of BeLLM. Subsequent sections are organized following the three steps outlined in the figure. Firstly, we introduce a degradation experiment to establish a turning point. Next, the proposed model is presented, including the Input Layer, LLM, and BiLLM. Lastly, contrastive learning for sentence embedding learning is introduced.

\subsection{Degradation Experiment}
\label{model::degradation}
Since we use prompt engineering to obtain the representative word of the sentence, the generation ability plays a crucial role. 
Typically, generation ability is associated with the number of layers in LLMs. 
LLMs with more layers tend to have a stronger generation ability \citep{kaplan2020scaling}.
We conduct a degradation experiment to explore the relationship between STS performance and the number of attention layers. 
Specifically, we systematically removed attention layers of LLMs from the last to the first and evaluated the model on the standard STS benchmark. 
The degradation results are shown in Figure \ref{figure_degradation}.
Notably, the results present a \textit{S}-shaped curve. This indicates overly strong and weak generation abilities fail to produce satisfactory STS performance. 
There is a turning point for generation ability in STS tasks. 
Once this turning point is exceeded, generation ability no longer positively impacts STS performance; instead, it becomes a negative factor, leading to a dramatic performance drop in the STS tasks. 
\textcolor{blue}{The figure clearly illustrates a noticeable turning point in all three models: ChatGLM-6B, LLaMA-7B, and LLaMA-13B. Interestingly, their turning points consistently occur at the penultimate layer.}
Supported by these findings, we convert attention layers after the turning point from uni- to bi-directional ones to introduce backward dependencies for improving STS.

\input{figure_degradation}


\subsection{Input Layer}
% 3.3 and 3.4 shares the Input Layer
We employ the tokenizer of the LLMs to derive input token indices. These indices are subsequently passed to the embedding layer of the LLMs to obtain word embeddings as follows:
 \begin{equation}
    \small
    \begin{split}
    \mathbf{x} &= \mathrm{Embedding}^{LLM}(t) \\
    t &= \mathrm{Tokenizer}^{LLM}(s),
    \end{split}
\end{equation}
where $s$ represents the input text.

\subsection{LLM}
We fetch the layers from the initial layer up to the layer at turning point $t$ from the LLMs, specifically denoted as $\mathrm{LLM}^{1:t}$. It keeps the autoregressive architecture and serves as the generation component of BeLLM.
Its attention computation is as follows:
\begin{equation}
    \small
    \mathrm{Attn}^{LLM}_i(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \mathrm{SoftMax}(\frac{\mathbf{Q}\mathbf{K}}{\sqrt{d}} + \mathcal{M}) \mathbf{V} 
\end{equation}
and
\begin{equation}
    \small
    \mathcal{M} = \begin{bmatrix}
     0 & -\infty & -\infty & -\infty & -\infty \\
     0 & 0 & -\infty  & -\infty & -\infty \\ 
     ... & ... & ... & ... & ...  \\ 
     0 & 0  & 0 & 0 &   -\infty \\
     0 & 0  & 0 & 0 & 0 
    \end{bmatrix},
\end{equation}
where $\mathrm{Attn}_i^{LLM}$ is the $i$-th head of multi-head self attention \citep{vaswani2017attention} in LLM. $\mathbf{Q} = \mathbf{W}^q\mathbf{x}+b$, $\mathbf{K} = \mathbf{W}^k\mathbf{x}+b$, $\mathbf{V} = \mathbf{W}^v\mathbf{x}+b$. $\mathcal{M}$ denotes the causal mask. It ensures that the $i$-th token is not visible to the $i+1...L$ tokens during attention computation, and $L$ is the input token length. 
%This is achieved because the values of $-\infty$ become zero after applying the softmax function.

These autoregressive layers can retain the generation ability. 
The generation ability is crucial for BeLLM since it uses prompt engineering to generate the representative word of the sentence.
Then, the embedding of the representative word is used as the sentence embedding. 
This approach can help to mitigate the \textit{anisotropy} problem \citep{ethayarajh-2019-contextual} caused by word frequency imbalance \citet{li-etal-2020-sentence}. 
This is because the representative word is usually not a high-frequency word. 
For example, a representative word for the sentence \textit{I am unhappy because it is raining.} obtained from LLaMA \citep{touvron2023llama2} is ``unhappy''. It is clearly not a high-frequency word such as ``it'', ``is'', or others. Specifically, we adopt the prompt \textit{The representative word for \{sentence\} is:"} to produce the representative word.

\subsection{BiLLM}
We detach the layers after turning point $t$ and transform them from uni- to bi-directional to obtain $\mathrm{BiLLM}^{t+1:n}$. Its attention is computed as follows:
\begin{equation}
    \small
    \mathrm{Attn}^{BiLLM}_i(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \mathrm{SoftMax}(\frac{\mathbf{Q}\mathbf{K}}{\sqrt{d}}) \mathbf{V},
\end{equation}
where $\mathbf{Q} = \mathbf{W}^q\mathbf{x}+b$, $\mathbf{K} = \mathbf{W}^k\mathbf{x}+b$, $\mathbf{V} = \mathbf{W}^v\mathbf{x}+b$.
By removing the causal mask, BeLLM is allowed to learn backward dependencies.

After obtaining the LLM and BiLLM components, the equation of BeLLM is as follows:
\begin{equation}
    \small
    \mathbf{h} = \mathrm{\overset{\rightarrow}{LLM}}^{1:t}(\mathbf{x}) + \mathrm{\overset{\rightleftarrows}{BiLLM}}^{t+1:n}(\mathbf{x}),
\end{equation}
where $\mathbf{x}$ is word embeddings. $t$ is the turning point. 

\subsection{Contrastive Learning}
We follow \citet{simcse_gao_2021} to optimize the contrastive objective to learn sentence embedding, as follows:
\begin{equation}
    \small
    \mathcal{L} = - \sum_i \mathrm{log} \frac{
        e^{cos(\mathbf{h}_i, \mathbf{h}_i^+)} / \tau
    }{
        \sum_{j=1}^N \left( 
            e^{cos(\mathbf{h}_i, \mathbf{h}_j^+) / \tau} + e^{cos(\mathbf{h}_i, \mathbf{h}_j^-) / \tau}
        \right) 
    },
\end{equation}
where $N$ is the mini-batch size, $\mathbf{h}_i^+$ and $\mathbf{h}_i^-$ refer to the positive and negative samples of $\mathbf{h}_i$, respectively. $\tau$ is the temperature. $cos(a, b)$ is the cosine similarity function. By employing contrastive learning, the embeddings of semantically similar sentences are pulled closer together, while those that are dissimilar are pushed apart.



==> table_case_study.old.tex <==
\begin{table*}[hbt!]
\centering
\setlength\tabcolsep{1.5pt}
\centering
\small
\begin{tabular}{llll}
\toprule
\multicolumn{2}{l}{\textbf{Query1}: A \textcolor{applegreen}{man} \textcolor{applegreen}{riding} a small \textcolor{applegreen}{boat} in a harbor.}                                                          & \multicolumn{2}{l}{\textbf{Query2}: A \textcolor{applegreen}{dog} \textcolor{applegreen}{runs} on the green \textcolor{applegreen}{grass} near a wooden \textcolor{applegreen}{fence}.}                                        \\ \midrule
\multicolumn{4}{c}{SimCSE$_{BERT}$}                                                                                                                                                                                                                          \\ \midrule
\multicolumn{1}{l}{\#1}                  & \multicolumn{1}{l}{A \textcolor{applegreen}{man} on a moored blue and white \textcolor{applegreen}{boat}.}                      & \multicolumn{1}{l}{\#1}                  & The \textcolor{applegreen}{dog} by the \textcolor{applegreen}{fence} is \textcolor{applegreen}{running} on the \textcolor{applegreen}{grass}.                              \\ 
\multicolumn{1}{l}{\#2}                  & \multicolumn{1}{l}{A \textcolor{applegreen}{man} is \textcolor{applegreen}{riding} in a \textcolor{applegreen}{boat} on the water.}                     & \multicolumn{1}{l}{\#2}                  & \textcolor{applegreen}{Dog} \textcolor{applegreen}{running} through \textcolor{applegreen}{grass} in \textcolor{applegreen}{fenced} area.                                  \\ 
\multicolumn{1}{l}{\#3}                  & \multicolumn{1}{l}{A \textcolor{applegreen}{man} in a blue \textcolor{applegreen}{boat} on the water.}                          & \multicolumn{1}{l}{\#3}                  & A \textcolor{applegreen}{dog} \textcolor{applegreen}{runs} on the green \textcolor{applegreen}{grass} near a grove of trees.                       \\ \midrule
\multicolumn{4}{c}{SimCSE$_{LLaMA}$}                                                                                                                                                                                                                            \\ \midrule
\multicolumn{1}{l}{\#1}                  & \multicolumn{1}{l}{A \textcolor{applegreen}{man} is \textcolor{applegreen}{riding} in a \textcolor{applegreen}{boat} on the water.}                     & \multicolumn{1}{l}{\#1}                  & The \textcolor{applegreen}{dog} by the \textcolor{applegreen}{fence} is \textcolor{applegreen}{running} on the \textcolor{applegreen}{grass}.                              \\
\multicolumn{1}{l}{\#2}                  & \multicolumn{1}{l}{A \textcolor{applegreen}{man} is \textcolor{applegreen}{operating} some type of vessel.}                     & \multicolumn{1}{l}{\#2}                  & A brown \textcolor{applegreen}{dog} \textcolor{applegreen}{runs} in the \textcolor{applegreen}{grass} with a wooden \textcolor{applegreen}{fence} behind.                  \\ 
\multicolumn{1}{l}{\#3}                  & \multicolumn{1}{l}{A \textcolor{applegreen}{man} in a blue \textcolor{applegreen}{boat} on the water.}                          & \multicolumn{1}{l}{\#3}                  & A \textcolor{applegreen}{dog} \textcolor{applegreen}{runs} on the green \textcolor{applegreen}{grass} near a grove of trees.                       \\ \midrule
\multicolumn{4}{c}{BeLLM}                                                                                                                                                                                                                            \\ \midrule
\multicolumn{1}{l}{\multirow{2}{*}{\#1}} & \multicolumn{1}{l}{A \textcolor{applegreen}{man} \textcolor{applegreen}{riding} a small \textcolor{applegreen}{boat} in a harbor,}                      & \multicolumn{1}{l}{\multirow{2}{*}{\#1}} & \multirow{2}{*}{A brown \textcolor{applegreen}{dog} \textcolor{applegreen}{runs} in the \textcolor{applegreen}{grass} with a wooden \textcolor{applegreen}{fence} behind.} \\ 
\multicolumn{1}{l}{}                     & \multicolumn{1}{l}{with fog and mountains in the background.}                   & \multicolumn{1}{l}{}                     &                                                                            \\ 
\multicolumn{1}{l}{\#2}                  & \multicolumn{1}{l}{A \textcolor{applegreen}{man} is \textcolor{applegreen}{riding} in a \textcolor{applegreen}{boat} on the water.}                     & \multicolumn{1}{l}{\#2}                  & The \textcolor{applegreen}{dog} by the \textcolor{applegreen}{fence} is \textcolor{applegreen}{running} on the \textcolor{applegreen}{grass}.                              \\ 
\multicolumn{1}{l}{\#3}                  & \multicolumn{1}{l}{A \textcolor{applegreen}{man} is \textcolor{applegreen}{floating} on a small \textcolor{applegreen}{boat} down a city water street.} & \multicolumn{1}{l}{\#3}                  & \textcolor{applegreen}{Dog} \textcolor{applegreen}{running} through \textcolor{applegreen}{grass} in \textcolor{applegreen}{fenced} in area.                               \\ \bottomrule
\end{tabular}
\caption{The top 3 retrieved sentences by SimCSE$_{BERT}$, SimCSE$_{LLaMA}$, and BeLLM from the Flickr30k dataset.}
\label{table_case_study}
\end{table*}

==> table_case_study.old2.tex <==
\begin{table*}[ht]
\small
\begin{tabular}{ll}
\toprule
\multicolumn{1}{l}{\textbf{Query}} & A \textcolor{applegreen}{female police officer} \textcolor{applegreen}{wears} an officer's \textcolor{applegreen}{hat} and \textcolor{applegreen}{sunglasses}.
\\ \midrule 
\multicolumn{2}{c}{\textbf{SimCSE$_{BERT}$}}                                                                                                                                                             \\ \midrule
\multicolumn{1}{l}{\#1}            & An officer stands next to a car on a city street.                                                                                                 \\ \midrule
\multicolumn{1}{l}{\#2}            & A \textcolor{applegreen}{police woman} smiling and \textcolor{applegreen}{wearing} \textcolor{applegreen}{sunglasses} and a \textcolor{applegreen}{hat}.                                                                                          \\ \midrule
\multicolumn{1}{l}{\multirow{2}{*}{\#3}} & \multicolumn{1}{l}{Young, smiling, blond \textcolor{applegreen}{female police officer} from New York}                                            \\ %\cline{2-2} 
\multicolumn{1}{l}{}                     & standing outside on a sidewalk. 
\\ \midrule
\multicolumn{2}{c}{\textbf{SimCSE$_{LLaMA}$}}                                                                                                                                                             \\ \midrule
\multicolumn{1}{l}{\multirow{2}{*}{\#1}} & \multicolumn{1}{l}{A \textcolor{applegreen}{female police officer} in a \textcolor{applegreen}{cap} and navy uniform smiles}                                             \\ %\cline{2-2} 
\multicolumn{1}{l}{}                     & while \textcolor{applegreen}{wearing sunglasses} outside of a shop.   \\ \midrule
\multicolumn{1}{l}{\multirow{2}{*}{\#2}} & \multicolumn{1}{l}{Young, smiling, blond \textcolor{applegreen}{female police officer} from New York}                                            \\ %\cline{2-2} 
\multicolumn{1}{l}{}                     & standing outside on a sidewalk. 
\\ \midrule
\multicolumn{1}{l}{\#3}            & An officer stands next to a car on a city street.                                                                                                 \\ \midrule
\multicolumn{2}{c}{\textbf{BeLLM}}                                                                                                                                                             \\ \midrule
\multicolumn{1}{l}{\multirow{2}{*}{\#1}} & \multicolumn{1}{l}{A \textcolor{applegreen}{female police officer} in a \textcolor{applegreen}{cap} and navy uniform smiles}                                             \\ %\cline{2-2} 
\multicolumn{1}{l}{}                     & while \textcolor{applegreen}{wearing} \textcolor{applegreen}{sunglasses} outside of a shop.
\\ \midrule
\multicolumn{1}{l}{\#2}            & A \textcolor{applegreen}{police woman} smiling and \textcolor{applegreen}{wearing} \textcolor{applegreen}{sunglasses} and a \textcolor{applegreen}{hat}.                                                                                          \\ \midrule
\multicolumn{1}{l}{\multirow{2}{*}{\#3}} & \multicolumn{1}{l}{Young, smiling, blond \textcolor{applegreen}{female police officer} from New York}                                            \\ %\cline{2-2} 
\multicolumn{1}{l}{}                     & standing outside on a sidewalk. 
\\ \bottomrule
\end{tabular}
\caption{The top 3 retrieved sentences by SimCSE$_{BERT}$, SimCSE$_{LLaMA}$, and BeLLM from the Flickr30k dataset.}
\label{table_case_study}
\end{table*}


==> table_case_study.old3.tex <==
\begin{figure*}
\CenterFloatBoxes
\begin{floatrow}
\ffigbox[\FBwidth]
{\caption{Visualization of forward and backward dependency graph of the query.}\label{figure_case_study}}
{
    \includegraphics[width=0.9\linewidth]{figures/case_study_dependency.pdf}
}
\killfloatstyle\ttabbox[\Xhsize]
{
\caption{The top 3 retrieved sentences by SimCSE$_{RoBERTa}$, SimCSE$_{LLaMA}$, and BeLLM from the Flickr30k dataset.}\label{table_case_study}}
{
    \small
    \setlength\tabcolsep{1.5pt}
    \begin{tabular}{ll}
    \toprule
    \multicolumn{1}{l}{\textbf{Q:}} & A \textcolor{applegreen}{female police officer} \textcolor{applegreen}{wears} an officer's \textcolor{applegreen}{hat} and \textcolor{applegreen}{sunglasses}.
    \\ \midrule 
    \multicolumn{2}{c}{SimCSE$_{RoBERTa}$}
    \\ \midrule
    \multicolumn{1}{l}{\#1}            & An officer stands next to a car on a city street.                                                                                                 \\ \midrule
    \multicolumn{1}{l}{\#2}            & A \textcolor{applegreen}{police woman} smiling and \textcolor{applegreen}{wearing} \textcolor{applegreen}{sunglasses} and a \textcolor{applegreen}{hat}.                                                                                          \\ \midrule
    \multicolumn{1}{l}{\multirow{2}{*}{\#3}} & \multicolumn{1}{l}{Young, smiling, blond \textcolor{applegreen}{female police officer} from New York}                                            \\ %\cline{2-2} 
    \multicolumn{1}{l}{}                     & standing outside on a sidewalk. 
    \\ \midrule
    \multicolumn{2}{c}{SimCSE$_{LLaMA}$}                                                                                                                                                             \\ \midrule
    \multicolumn{1}{l}{\multirow{2}{*}{\#1}} & \multicolumn{1}{l}{A \textcolor{applegreen}{female police officer} in a \textcolor{applegreen}{cap} and navy uniform smiles}                                             \\ %\cline{2-2} 
    \multicolumn{1}{l}{}                     & while \textcolor{applegreen}{wearing sunglasses} outside of a shop.   \\ \midrule
    \multicolumn{1}{l}{\multirow{2}{*}{\#2}} & \multicolumn{1}{l}{Young, smiling, blond \textcolor{applegreen}{female police officer} from New York}                                            \\ %\cline{2-2} 
    \multicolumn{1}{l}{}                     & standing outside on a sidewalk. 
    \\ \midrule
    \multicolumn{1}{l}{\#3}            & An officer stands next to a car on a city street.                                                                                                 \\ \midrule
    \multicolumn{2}{c}{BeLLM}                                                                                                                                                             \\ \midrule
    \multicolumn{1}{l}{\multirow{2}{*}{\#1}} & \multicolumn{1}{l}{A \textcolor{applegreen}{female police officer} in a \textcolor{applegreen}{cap} and navy uniform smiles}                                             \\ %\cline{2-2} 
    \multicolumn{1}{l}{}                     & while \textcolor{applegreen}{wearing} \textcolor{applegreen}{sunglasses} outside of a shop.
    \\ \midrule
    \multicolumn{1}{l}{\#2}            & A \textcolor{applegreen}{police woman} smiling and \textcolor{applegreen}{wearing} \textcolor{applegreen}{sunglasses} and a \textcolor{applegreen}{hat}.                                                                                          \\ \midrule
    \multicolumn{1}{l}{\multirow{2}{*}{\#3}} & \multicolumn{1}{l}{Young, smiling, blond \textcolor{applegreen}{female police officer} from New York}                                            \\ %\cline{2-2} 
    \multicolumn{1}{l}{}                     & standing outside on a sidewalk. 
    \\ \bottomrule
    \end{tabular}
}
\end{floatrow}
\end{figure*}

==> table_case_study.single_column.tex <==
\begin{table}[]
\small
\setlength\tabcolsep{1pt}
\begin{tabular}{ll}
\midrule
\textbf{Q1:}                                         & \multicolumn{1}{l}{\textbf{A man riding a small boat in a harbor.}}                                                 \\ \midrule
\multicolumn{2}{c}{SimCSE}                                                                                                                   \\ \midrule
\multicolumn{1}{l}{\#1}                   & \multicolumn{1}{l}{A man on a moored blue and white boat.}               \\ \midrule
\multicolumn{1}{l}{\#2}                   & \multicolumn{1}{l}{A man is riding in a boat on the water.}                                     \\ \midrule
\multicolumn{1}{l}{\#3}                   & \multicolumn{1}{l}{A man in a blue boat on the water.}                                          \\ \midrule
\multicolumn{2}{c}{LLaMA}                                                                                                                    \\ \midrule
\multicolumn{1}{l}{\#1}                   & \multicolumn{1}{l}{A man is riding in a boat on the water.}                                     \\ \midrule
\multicolumn{1}{l}{\#2}                   & \multicolumn{1}{l}{A man is operating some type of vessel.}                                     \\ \midrule
\multicolumn{1}{l}{\#3}                   & \multicolumn{1}{l}{A man in a blue boat on the water.}                                          \\ \midrule
\multicolumn{2}{c}{BeLLM}                                                                                                                    \\ \midrule
\multicolumn{1}{l}{}                      & \multicolumn{1}{l}{A man riding a small boat in a harbor, with fog and}                                      \\ %\cline{2-2} 
\multicolumn{1}{l}{\multirow{-2}{*}{\#1}} & \multicolumn{1}{l}{mountains in the background.}                                   \\ \midrule
\multicolumn{1}{l}{\#2}                   & \multicolumn{1}{l}{A man is riding in a boat on the water.}                                     \\ \midrule
\multicolumn{1}{l}{}                   & \multicolumn{1}{l}{A man is floating on a small boat down }    \\             
\multicolumn{1}{l}{\multirow{-2}{*}{\#3}} & \multicolumn{1}{l}{a city water street.}                                 
\\ \midrule
\midrule
\textbf{Q2:}                                         & \multicolumn{1}{l}{\textbf{A dog runs on the green grass near a wooden fence.}}                                                 \\ \midrule
\multicolumn{2}{c}{SimCSE}                                                                                                                   \\ \midrule
\multicolumn{1}{l}{\#1}                   & \multicolumn{1}{l}{The dog by the fence is running on the grass.}                               \\ \midrule
\multicolumn{1}{l}{\#2}                   & \multicolumn{1}{l}{Dog running through grass in fenced area.}                                   \\ \midrule
\multicolumn{1}{l}{\#3}                   & \multicolumn{1}{l}{A dog runs on the green grass near a grove of trees.}                        \\ \midrule
\multicolumn{2}{c}{LLaMA}                                                                                                                    \\ \midrule
\multicolumn{1}{l}{\#1}                   & \multicolumn{1}{l}{The dog by the fence is running on the grass.}                               \\ \midrule
\multicolumn{1}{l}{}                      & \multicolumn{1}{l}{A brown dog runs in the grass with a wooden }                                      \\ %\cline{2-2} 
\multicolumn{1}{l}{\multirow{-2}{*}{\#2}} & \multicolumn{1}{l}{fence behind.}                                   \\ \midrule
\multicolumn{1}{l}{\#3}                   & \multicolumn{1}{l}{A dog runs on the green grass near a grove of trees.}                        \\ \midrule
\multicolumn{2}{c}{BeLLM}                                                                                                                    \\ \midrule
\multicolumn{1}{l}{}                      & \multicolumn{1}{l}{A brown dog runs in the grass with a wooden }                                      \\ %\cline{2-2} 
\multicolumn{1}{l}{\multirow{-2}{*}{\#2}} & \multicolumn{1}{l}{ fence behind.}                                   \\ \midrule
\multicolumn{1}{l}{\#2}                   & \multicolumn{1}{l}{The dog by the fence is running on the grass.}                               \\ \midrule
\#3                                         & Dog running through grass in fenced in area.                                                     \\ \midrule
\end{tabular}
\caption{The top 3 retrieved sentences by BERT, LLaMA, and BeLLM from the Flickr30k dataset.}
\label{table_case_study}
\end{table}

==> table_csts.old.tex <==
\begin{table}[ht]
\small
\centering
\begin{threeparttable}
\begin{tabular}{lc}
\toprule
Model & Spearman's \\
\midrule
\midrule
Flan-T5$_{XL}$ $\dagger$  & $24.80$ \\
Flan-T5$_{XXL}$ $\dagger$  & $29.20$ \\
Flan-UL2 $\dagger$  & $23.20$ \\
Tk-Instruct$_{3B}$ $\dagger$  & $4.90$ \\
Tk-Instruct$_{11B}$ $\dagger$  & $17.10$ \\
GPT-3.5 $\dagger$ & $15.50$ \\
GPT-4  $\dagger$ & $43.60$ \\
\midrule
\textbf{SimCSE}\\
+RoBERTa$_{large}$ (previous SOTA) $\dagger$ & $47.50$ \\
% \midrule
% \multicolumn{2}{c}{\textit{Ours}} \\
% \midrule
+LLaMA & $48.64\ \  \scalebox{0.65}{\color{red} +1.14\%}$  \\
+BeLLM (ours) & $\mathbf{49.74}\ \scalebox{0.65}{\color{red}+2.24\%}$ \\

\bottomrule
\end{tabular}
\end{threeparttable}
\caption{Results on the C-STS test set. The metrics are Spearman's correlation, which is computed using the official C-STS test API. $\dagger$ denotes results are retrieved from \cite{deshpande2023csts}. LLM baselines are evaluated in few-shot settings.}
\label{table::csts}
\end{table}

==> table_csts_example.old.tex <==
\begin{table*}[]
\small
\setlength\tabcolsep{1.5pt}
\centering
\begin{tabular}{lll}
\toprule
\multicolumn{1}{c}{\textbf{Sentence 1}}  & \multicolumn{1}{c}{\textbf{Sentence 2}}  & \multicolumn{1}{c}{\textbf{Condition and Similarity}} \\ 
\midrule
\multirow{1}{*}{
    \begin{tabular}[c]{@{}l@{}}
     An older man holding a glass\\ of wine while standing between \\  two beautiful ladies.
    \end{tabular}
} & 
\multirow{1}{*}{
    \begin{tabular}[c]{@{}l@{}}
        A group of people gather\\   around a table with bottles\\   and glasses of wine.
    \end{tabular}
}& 
The people’s demeanor: $5$ \\[1ex]
\cline{3-3} \\[-1.8ex]& & The number of bottles: $1$  \\[0.5ex]
\bottomrule
\end{tabular}
\caption{An example from the C-STS validation set, where the same sentence pair has different similarities based on different conditions. A similarity score of 1 indicates dissimilar, while a score of 5 represents similar.}
\label{table_csts_example}
\end{table*}

==> table_standard_sts.old.tex <==
\begin{table*}[ht]
\setlength\tabcolsep{1.5pt}
\small
\centering
\begin{threeparttable}
\begin{tabular}{lcccccccc}
\toprule
Model & STS12 & STS13 & STS14 & STS15 & STS16 & STS-B & SICR-R & Avg. \\

\midrule
\midrule
\multicolumn{9}{c}{\textit{Closed Models}} \\
\midrule
% text-embedding-ada-002
openai-ada-002 $\diamondsuit$ & $69.80$ & $83.27$ & $76.09$  & $86.12$  & $85.96$  & $83.17$   & $80.60$ & $80.72$ \\ 


\midrule
\midrule
\multicolumn{9}{c}{\textit{Unsupervised Models}} \\

\midrule
GloVe (avg.) $\dagger$ & $55.14$ & $70.66$ & $59.73$  & $68.25$  & $63.66$  & $58.02$   & $53.76$ & $61.32$ \\ 
\textbf{BERT} \\
+flow $\ddagger$ & $58.40$ & $67.10$ & $60.85$  & $75.16$  & $71.22$  & $68.66$   & $64.47$ & $66.55$ \\
+whitening $\ddagger$ & $57.83$ & $66.90$ & $60.90$  & $75.08$  & $71.31$  & $68.24$   & $63.73$ & $66.28$ \\
+IS $\ddagger$ & $56.77$ & $69.24$ & $61.21$ & $75.23$ & $70.16$ & $69.21$ & $64.25$ & $66.58$ \\
+CT $\ddagger$ & $61.63$ & $76.80$ & $68.47$ & $77.50$ & $76.48$ & $74.31$ & $69.19$ & $72.05$ \\
+ConSERT & $64.64$ & $78.49$ & $69.07$ & $79.72$ & $75.95$ & $73.97$ & $67.31$ & $72.74$ \\
+DiffCSE & $72.28$ & $84.43$ & $76.47$ & $83.90$ & $80.54$ & $80.59$ & $71.23$ & $78.49$ \\
+SimCSE  & $68.40$ & $82.41$ & $74.38$ & $80.91$ & $78.56$ & $76.85$ & $72.23$ & $76.25$ \\
% LLaMA2-7B $\star$ & $50.66$ & $73.32$ & $62.76$ & $67.00$ & $70.98$ & $63.28$ & $67.40$ & $65.06$ \\

\midrule
\midrule
\multicolumn{9}{c}{\textit{Supervised Models}} \\
\midrule

InferSent $\dagger$  & $52.86$ & $66.75$ & $62.15$ & $72.77$ & $66.87$ & $68.03$ & $65.65$ & $65.01$ \\
USE $\dagger$ & $64.49$ & $67.80$ & $64.61$ & $76.83$ & $73.18$ & $74.92$ & $76.69$ & $71.22$ \\
ConSERT & $74.07$ & $83.93$ & $77.05$ & $83.66$ & $78.76$ & $81.36$ & $76.77$ & $79.37$ \\
SBERT $\dagger$ & $70.97$ & $76.53$ & $73.19$ & $79.09$ & $74.30$ & $77.03$ & $72.91$ & $74.89$ \\
\midrule
\textbf{SimCSE} \\
+RoBERT$_{large}$ & $77.46$ & $87.27$ & $82.36$ & $86.66$ & $83.93$ & $86.70$ & $\mathbf{81.95}$ & $83.76$ \\
+LLaMA $\clubsuit$ & $78.39\  \scalebox{0.65}{\color{red} +0.93\%}$ & $89.95\  \scalebox{0.65}{\color{red} +2.68\%}$ & $84.80\  \scalebox{0.65}{\color{red} +2.44\%}$ & $88.50\  \scalebox{0.65}{\color{red} +1.84\%}$ & $86.04\  \scalebox{0.65}{\color{red} +2.11\%}$ & $87.86\  \scalebox{0.65}{\color{red} +1.16\%}$ & $81.11\  \scalebox{0.65}{\color{applegreen} -0.84\%}$ & $85.24\  \scalebox{0.65}{\color{red} +1.48\%}$ \\ 
+BeLLM & $79.39\  \scalebox{0.65}{\color{red} +1.93\%}$ & $\mathbf{91.04}\  \scalebox{0.65}{\color{red} +3.77\%}$ & $\mathbf{86.52}\  \scalebox{0.65}{\color{red} +4.16\%}$ & $89.24\  \scalebox{0.65}{\color{red} +2.58\%}$ & $\mathbf{87.43}\  \scalebox{0.65}{\color{red} +3.50\%}$ & $\mathbf{89.04}\  \scalebox{0.65}{\color{red} +2.34\%}$ & $81.14\  \scalebox{0.65}{\color{applegreen} -0.81\%}$ & $\mathbf{86.26}\  \scalebox{0.65}{\color{red} +2.50\%}$ \\ 

\bottomrule
\end{tabular}
\end{threeparttable}
\caption{Sentence embedding performance on STS tasks. We report the Spearman's correlation $\rho \times 100$ of the ``all'' setting computed by SentEval \citep{conneau-kiela-2018-senteval}. Results marked with $\dagger$ are obtained from \citep{sbert-nils-2019}, while results marked with $\ddagger$ are retrieved from \citep{simcse_gao_2021}. The model marked with $\diamondsuit$ represents the embedding model released by OpenAI, and its results are obtained from \citep{muennighoff2022mteb}. Additionally, results marked with $\clubsuit$ are retrieved from \citep{li2023angle}. We refer to the corresponding original papers for the remaining baselines to obtain their results.}
\label{table::main}
\end{table*}

==> table_transfer.old.tex <==
\begin{table*}[ht]
\setlength\tabcolsep{1.5pt}
\small
\centering
\begin{threeparttable}
\begin{tabular}{lcccccccc}
\toprule
Model & MR & CR & SUBJ & MPQA & SST2 & TREC & MRPC & Avg. \\

\midrule
\midrule

GloVe $\dagger$ & $77.25$ & $78.30$ &  $91.17$ &  $87.85$ & $80.18$ &  $83.00$ & $72.87$ &  $81.52$ \\ 
Skip-thought $\ddagger$ & $76.50$ & $80.10$ & $93.60$ & $87.10$ &  $82.00$ & $92.20$ & $73.00$ & $83.50$ \\
\midrule

Avg. BERT $\dagger$ & $78.66$ & $86.25$ & $94.37$ & $88.66$ &  $84.40$ & $92.80$ & $69.54$ & $84.94$ \\

BERT-CLS $\dagger$ & $78.68$ & $84.85$ & $94.21$ & $88.23$ & $84.13$ & $91.40$ & $71.13$ & $84.66$ \\

IS-BERT $\ddagger$ & $81.09$ & $87.18$ & $94.96$ & $88.75$ & $85.96$  & $88.64$ & $74.24$ &  $85.83$ \\

DiffCSE $\diamondsuit$ & $82.82$ & $88.61$ & $94.32$ & $87.71$ & $88.63$ & $90.40$ & $\mathbf{76.81}$ & $87.04$ \\
\midrule
\textbf{SimCSE} \\
+RoBERTa $\star$ & $83.37$ & $87.76$ & $95.05$ & $87.16$ & $89.02$ & $90.80$ & $75.13$ &  $86.90$ \\
+LLaMA $\clubsuit$ & $90.40\  \scalebox{0.65}{\color{red} +7.03\%}$ & $92.90\  \scalebox{0.65}{\color{red} +5.14\%}$ & $\mathbf{96.88}\  \scalebox{0.65}{\color{red} +1.83\%}$ & $91.57\  \scalebox{0.65}{\color{red} +4.41\%}$ & $95.11\  \scalebox{0.65}{\color{red} +6.09\%}$ & $95.40\  \scalebox{0.65}{\color{red} +4.60\%}$ & $75.13\  \scalebox{0.65}{+0.00\%}$ & $91.06\  \scalebox{0.65}{\color{red} +4.16\%}$ \\
+BeLLM & $\mathbf{90.79}\  \scalebox{0.65}{\color{red} +7.42\%}$ & $\mathbf{93.43}\  \scalebox{0.65}{\color{red} +5.67\%}$ & $96.53\  \scalebox{0.65}{\color{red} +1.48\%}$ & $\mathbf{92.01}\  \scalebox{0.65}{\color{red} +4.85\%}$ & $\mathbf{95.77}\  \scalebox{0.65}{\color{red} +6.75\%}$ & $\mathbf{95.45}\  \scalebox{0.65}{\color{red} +4.65\%}$ & $\mathbf{75.48}\  \scalebox{0.65}{\color{red} +0.35\%}$ & $\mathbf{91.35}\  \scalebox{0.65}{\color{red} +4.45\%}$ \\

\bottomrule

\end{tabular}
\end{threeparttable}
\caption{Transfer task results of different sentence embedding models (measured as accuracy). $\dagger$: results from \citet{sbert-nils-2019}; $\ddagger$: results from \citet{zhang-etal-2020-unsupervised}; $\star$: results from \citet{simcse_gao_2021}. $\diamondsuit$: results from \citet{chuang-etal-2022-diffcse}; $\clubsuit$: results from \citet{jiang2023scaling}; % $\spadesuit$: results from \citet{li2023angle}.
}
\label{table::transfer}
\end{table*}

